Introducing Depth into Transformer-based 3D Object Detection

In this paper, we present DAT, a Depth-Aware Transformer framework designed for camera-based 3D detection. Our model is based on observing two major issues in existing methods: large depth translation errors and duplicate predictions along depth axes. To mitigate these issues, we propose two key solutions within DAT. To address the first issue, we introduce a Depth-Aware Spatial Cross-Attention (DA-SCA) module that incorporates depth information into spatial cross-attention when lifting image features to 3D space. To address the second issue, we introduce an auxiliary learning task called Depth-aware Negative Suppression loss. First, based on their reference points, we organize features as a Bird's-Eye-View (BEV) feature map. Then, we sample positive and negative features along each object ray that connects an object and a camera and train the model to distinguish between them. The proposed DA-SCA and DNS methods effectively alleviate these two problems. We show that DAT is a versatile method that enhances the performance of all three popular models, BEVFormer, DETR3D, and PETR. Our evaluation on BEVFormer demonstrates that DAT achieves a significant improvement of +2.8 NDS on nuScenes val under the same settings. Moreover, when using pre-trained VoVNet-99 as the backbone, DAT achieves strong results of 60.0 NDS and 51.5 mAP on nuScenes test. Our code will be soon.

==> figs/motivation.tex <==
\begin{figure}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/motivation_no_dpt.pdf}
    \caption{An illustration of a common ambiguity problem in DETR-based 3D detectors. $AC$ is a ray pointing from an object center $A$ to a camera $C$. The yellow ray is the projection of the object ray $AC$ on the BEV plane. Note that 3D reference points $r1$, $r2$, and $r3$ will be mapped to the same camera reference point.
    % According to the rule BEVFormer maps 3D points to camera space, all reference points ($r^1, r^2, r^3$) on the extension line of $AC$ will be mapped to the same position. 
    The car drawn with a solid line at $r^2$ denotes the GT center of the object, whereas the ones with dash lines at $r^1$ and $r^3$ means the object is not in these positions, but detection head will ``see'' an object there. The green cell denotes the BEV feature at the GT center and the red cells denote BEV features at pseudo-GT centers.}
    \label{fig:motivation bevformer}
\end{figure}


==> figs/tex_SCA_compare.tex <==
\begin{figure*}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/sca.pdf}
    \caption{The comparison between DA-SCA and SCA in previous works. PETR adopts standard attention. They include positional encoding of $(x, y, z)$ in both queries and keys. For keys, they do not have $d$, so they sample $d$ uniformly along the depth direction in a valid scope and sum up all the positional encodings of converted $(x, y, z)$ over all $d$'s, we use $\Bar{d}$ to indicate that they do not have informative depth. DETR3D and BEVFormer adopt deformable attention without using keys. They use a $(u, v)$ reference point to guide where to query features from and add positional encoding of $(x, y, z)$ to the content part of a query for predicting deformable sampling points. They all neglect the depth information in SCA. By contrast, DA-SCA adopts $(u, v, d)$ positional encoding in both image features and queries.}
    \label{fig:sca}
\end{figure*}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> sec/todo.tex <==
%1. fig1 c蓝色改醒目的颜色（金黄），绿色箭头改橙色试试；supervision -> learning
%2. fig2: (a)->(b), (b)也要加类似的两根线；（a)highlight redundant red boxes


==> tables/ablation_imp_obj.tex <==
\begin{table*}
% \vspace{-2mm}
% \resizebox{0.9\textwidth}{!}{
\centering
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{l|c|cccccc|c}
\toprule
\textbf{Method}                                   & \textbf{Modality} & \textbf{mAP}$\uparrow$  & \textbf{mATE}$\downarrow$ & \textbf{mASE}$\downarrow$  & \textbf{mAOE}$\downarrow$ & \textbf{mAVE}$\downarrow$ & \textbf{mAAE}$\downarrow$ & \textbf{NDS}$\uparrow$ \\
\midrule
Implicit object level                                & C        & - & - & - & -   & - & - & 0.539  \\
Explicit object level                                & C        & - & - & - & -   & - & - & -  \\
Explicit pixel level                                & C        & - & - & - & -   & - & - & -  \\
\bottomrule
\end{tabular}% }
\caption{Effectiveness of implicit object-level depth learning.}

\label{tab:test}
\end{table*}

==> tables/explicit.tex <==
\begin{table*}[t]
% \vspace{-2mm}
% \resizebox{0.9\textwidth}{!}{
\centering
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{c|l|c|cccccc|c}
\toprule
\textbf{Row}&
\textbf{Method}                                   & \textbf{Modality} & \textbf{mAP}$\uparrow$  & \textbf{mATE}$\downarrow$ & \textbf{mASE}$\downarrow$  & \textbf{mAOE}$\downarrow$ & \textbf{mAVE}$\downarrow$ & \textbf{mAAE}$\downarrow$ & \textbf{NDS}$\uparrow$ \\
\midrule
% 1.&BEVFormer      & C        & 0.416 & 0.673 & 0.274 & 0.372   & 0.394 & 0.198 & 0.517  \\
1.&BEVFormer+DA-SCA                                 & C        & 0.420 & 0.663 & 0.269 & 0.377   & 0.359 & 0.185 & 0.525 \\
2.&Row1+object-level loss                                & C    & 0.427 & 0.668 & 0.271 & 0.378   & 0.354 & 0.205 & 0.526  \\
3.&Row1+pixel-level loss                                & C    & 0.419 & 0.660 & 0.272 & 0.345   & 0.353 & 0.189 & 0.527  \\
4.&Row1+\sdcl                               & C    & 0.428 & 0.633 & 0.273 & 0.331   & 0.327 & 0.188 & 0.539  \\
% DG-BEV-S     & C    & 1312    & 0.428 & 0.633 & 0.273 & 0.331   & 0.327 & 0.188 & 0.539  \\
% DG-BEV     & C    & 1323    & \textbf{0.433} & 0.623 & 0.271 & 0.351   & 0.309 & 0.188 & \textbf{0.545} 
\bottomrule
\end{tabular}% }
\caption{The results of two explicit depth learning methods comparing with our \dcl.}

\label{tab:appendix:explicit}
\end{table*}
